Taylor rolls on tour: Slow drift of turbulent large-scale structures in flows with continuous symmetries

In Rayleigh-Benard convection and Taylor-Couette flow cellular patterns emerge at the onset of instability and persist as large-scale coherent structures in the turbulent regime. Their long-term dynamics has been thoroughly characterised and modelled for the case of turbulent convection, whereas turbulent Taylor rolls have received much less attention. Here we present direct numerical simulations of axisymmetric Taylor-Couette flow and show a discontinuous phase-transition to spatio-temporal chaos as the system size increases. Beyond this transition, Taylor rolls suddenly undergo erratic drifts evolving on a very slow time scale. We estimate an effective diffusion coefficient for the drift and compare the dynamics to analogous motions in Rayleigh-Benard convection and Poiseuille flow, suggesting that this spontaneous diffusive displacement of large coherent structures is common among different types of wall-bounded turbulent flows.

==> userDefs/myCommands.tex <==
\RequirePackage{xspace}   % to get your spacing straight

%--- special characters -------------------------------------------------------%
\DeclareRobustCommand{\increment}{\,d\!}
\DeclareRobustCommand{\imag}{\ensuremath{\dot{\imath}}\xspace}  % imaginary unit
\DeclareRobustCommand{\orderof}[1]{\ensuremath{\mathcal{O}\!\left(#1\right)}\xspace}     % magnitude
\DeclareRobustCommand{\real}{\ensuremath{\mathcal{R}}\xspace}        % real part

% statistical average delimiter
\DeclareRobustCommand{\lla}{\left\langle}
\DeclareRobustCommand{\rra}{\right\rangle}

% text subscripts
\DeclareRobustCommand{\analytical}{\text{ana}}
\DeclareRobustCommand{\bulk}{\text{b}}
\DeclareRobustCommand{\characteristic}{c\!h\!a}
\DeclareRobustCommand{\constant}{\text{const}}
\DeclareRobustCommand{\critical}{\text{krit}}
\DeclareRobustCommand{\initial}{i\!n\!i}
\DeclareRobustCommand{\numerical}{n\!u\!m}
\DeclareRobustCommand{\reference}{\text{ref}}
\DeclareRobustCommand{\tidal}{t\!i\!d}

% special variables
\DeclareRobustCommand{\ubulk}{\ensuremath{u_{\bulk}}\xspace}          % bulk velocity
\DeclareRobustCommand{\uhpc}{\ensuremath{u_{\text{c,HP}}}\xspace}     % Hagen-Poiseuille center line
\DeclareRobustCommand{\uref}{\ensuremath{u_{\reference}}\xspace}      % reference velocity
\DeclareRobustCommand{\oref}{\ensuremath{\omega_{\reference}}\xspace} % reference angular velocity
\DeclareRobustCommand{\nsym}{\ensuremath{n_{\text{sym}}}\xspace}      % n-fold symmetry
\DeclareRobustCommand{\tauw}{\ensuremath{\tau_{\text{w}}}\xspace}     % wall shear stress
\DeclareRobustCommand{\utau}{\ensuremath{u_{\tau}}\xspace}          % friction velocity

% non-dimensional numbers
\DeclareRobustCommand{\Courant}{\ensuremath{C\!o}\xspace} % Courant number
\DeclareRobustCommand{\Mach}{\ensuremath{M\!a}\xspace} % Mach number
\DeclareRobustCommand{\Nusselt}{\ensuremath{N\hspace{-0.20em}u}\xspace} % Nusselt number
\DeclareRobustCommand{\Nui}{\ensuremath{N\hspace{-0.27em}u_{i}}\xspace} % inner Nusselt number
\DeclareRobustCommand{\Nuo}{\ensuremath{N\hspace{-0.27em}u_{o}}\xspace} % outer Nusselt number
\DeclareRobustCommand{\Nuomi}{\ensuremath{N\hspace{-0.27em}u_{\omega,i}}\xspace}
\DeclareRobustCommand{\Nuomo}{\ensuremath{N\hspace{-0.27em}u_{\omega,o}}\xspace}
\DeclareRobustCommand{\NuS}{\ensuremath{N\hspace{-0.20em}u_{\hspace{-0.1em}s}}\xspace} % shear Nusselt number
\DeclareRobustCommand{\NuT}{\ensuremath{N\hspace{-0.27em}u_{T}}\xspace} % thermal Nusselt number
\DeclareRobustCommand{\Prandtl}{\ensuremath{P\hspace{-0.1em}r}\xspace}  % Prandtl number
\DeclareRobustCommand{\Rayleigh}{\ensuremath{R\hspace{-0.1em}a}\xspace} % Rayleigh number
\DeclareRobustCommand{\Reynolds}{\ensuremath{R\hspace{-0.1em}e}\xspace} % Reynolds number
\DeclareRobustCommand{\ReDelta}{\ensuremath{R\hspace{-0.1em}e_{\delta}}\xspace}
\DeclareRobustCommand{\Rei}{\ensuremath{R\hspace{-0.1em}e_{i}}\xspace} % inner Reynolds number
\DeclareRobustCommand{\Reo}{\ensuremath{R\hspace{-0.1em}e_{o}}\xspace} % outer Reynolds number
\DeclareRobustCommand{\Romega}{\ensuremath{R_{\omega}}\xspace}         % rotation number

\DeclareRobustCommand{\ROmega}{\ensuremath{R_{\Omega}}\xspace}         % rotation number
\DeclareRobustCommand{\ReS}{\ensuremath{R\hspace{-0.1em}e_{\hspace{-0.1em}s}}\xspace} % shear Reynolds number

\DeclareRobustCommand{\ROmegaDub}{\ensuremath{R^{\ast}_{\Omega}}\xspace}         % rotation number
\DeclareRobustCommand{\ReSDub}{\ensuremath{R\hspace{-0.1em}e^{\ast}_{S}}\xspace} % shear Reynolds number
\DeclareRobustCommand{\NuSDub}{\ensuremath{N\hspace{-0.27em}u^{\ast}_{S}}\xspace} % shear Nusselt number
\DeclareRobustCommand{\NuTDub}{\ensuremath{N\hspace{-0.27em}u^{\ast}_{T}}\xspace} % thermal Nusselt number

\DeclareRobustCommand{\ReTau}{\ensuremath{R\hspace{-0.1em}e_{\tau}}\xspace}
\DeclareRobustCommand{\Strouhal}{\ensuremath{S\!t}\xspace}   % Strouhal number
\DeclareRobustCommand{\Taylor}{\ensuremath{T\hspace{-0.3em}a}\xspace} % Taylor number
\DeclareRobustCommand{\Womersley}{\ensuremath{W\!o}\xspace}   % Womersley number

\DeclareRobustCommand{\RBC}{Rayleigh--B\'enard convection\xspace}
\DeclareRobustCommand{\TCF}{Taylor--Couette flow\xspace}

% special math functions
\DeclareRobustCommand{\Bessel}{\ensuremath{\mathcal{J}_{0}}\xspace}   % Bessel function of first kind and order zero

% vector operators
\renewcommand{\vec}{\boldsymbol}
\DeclareRobustCommand{\divergence}{\operatorname{div}}
\DeclareRobustCommand{\gradient}{\operatorname{grad}}
\RequirePackage{rotating} % provides sideways
\DeclareRobustCommand{\laplacian}{\vec{\Delta}}
\renewcommand{\nabla}{\begin{sideways}\begin{sideways}$\laplacian$\end{sideways}\end{sideways}}

% relations
\DeclareRobustCommand{\constraint}{\stackrel{!}{=}}

% some software names
\RequirePackage{xspace}
\RequirePackage{hyperref}
\DeclareRobustCommand{\code}[1]{\textbf{\texttt{\color{black}#1}}\xspace}
\DeclareRobustCommand{\hdf}{\href{https://en.wikipedia.org/wiki/Hierarchical_Data_Format}{\code{HDF5}}\xspace}
\DeclareRobustCommand{\mpi}{\href{https://en.wikipedia.org/wiki/Message_Passing_Interface}{\code{MPI}}\xspace}
\DeclareRobustCommand{\nsc}{\href{https://github.com/dfeldmann/nsCouette}{\code{nsCouette}}\xspace}
\DeclareRobustCommand{\tlab}{\href{https://github.com/turbulencia/Tlab}{\code{tLab}}\xspace}
\DeclareRobustCommand{\omp}{\href{https://en.wikipedia.org/wiki/OpenMP}{\code{OpenMP}}\xspace}
\DeclareRobustCommand{\python}{\href{https://www.python.org/}{\code{Python}}\xspace}
\DeclareRobustCommand{\spp}{\href{https://gepris.dfg.de/gepris/projekt/273183002?language=en}{\texttt{Turbulent Superstructures (SPP1881)}}\xspace}
\DeclareRobustCommand{\hlrn}{\href{https://www.hlrn.de/?lang=en}{North German Supercomputing Alliance (HLRN)}\xspace}
\DeclareRobustCommand{\pangaea}{\href{https://www.pangaea.de/}{Pangaea}\xspace}


% common abbreviations
\DeclareRobustCommand{\cf}{c.\,f.\xspace}
\DeclareRobustCommand{\eg}{e.\,g.\xspace}
\DeclareRobustCommand{\Eg}{E.\,g.\xspace}
\DeclareRobustCommand{\etc}{etc.\xspace}
\DeclareRobustCommand{\ie}{i.\,e.\xspace}
\DeclareRobustCommand{\Ie}{I.\,e.\xspace}
\DeclareRobustCommand{\wrt}{w.\,r.\,t.\xspace}

% draft stage
\DeclareRobustCommand{\mod}[1]{{\color{Vermillion}#1}} % \xspace
\DeclareRobustCommand{\ak}[1]{{\color{Vermillion}(\textbf{AK}: \textit{#1})}\xspace}
\DeclareRobustCommand{\df}[1]{{\color{Vermillion}(\textbf{DF}: \textit{#1})}\xspace}
\DeclareRobustCommand{\ma}[1]{{\color{Vermillion}(\textbf{MA}: \textit{#1})}\xspace}
\DeclareRobustCommand{\todo}[1]{{\color{Vermillion}(\textbf{To do}: \textit{#1})}\xspace}
\DeclareRobustCommand{\q}[1]{{\color{Vermillion}(\textbf{Question}: \textit{#1})}\xspace}

\DeclareRobustCommand{\Editor}{\item[{\color{Vermillion}Edit.}]\color{Grey}}
\DeclareRobustCommand{\RefereeA}{\item[{\color{Vermillion}Ref. A}]\color{Grey}}
\DeclareRobustCommand{\RefereeB}{\item[{\color{Vermillion}Ref. B}]\color{Grey}}
\DeclareRobustCommand{\Response}{\item[{\color{Blue}Resp.}]\color{Black}}


==> userDefs/myPreamble.tex <==
% font encoding
% \usepackage[T1]{fontenc}    % output
% \usepackage[utf8]{inputenc} % input
% \RequirePackage{url}        % to avoid probs with special chars in email or web address

% language settings
% \usepackage[UKenglish]{babel}

\usepackage{pifont}

% math, units and numbers
\usepackage{bm} % bold math
\RequirePackage{amsmath}
\RequirePackage{amssymb}
\RequirePackage{amstext}
\RequirePackage{dsfont}
\RequirePackage{xfrac}
\RequirePackage{siunitx}
\sisetup{tight-spacing=true}
\sisetup{print-unity-mantissa=false}
\PassOptionsToPackage{decimalsymbol=.}{siunitx}


% figures
% \RequirePackage{graphicx}
% \RequirePackage{overpic}
% \RequirePackage{epsfig}
% \RequirePackage{float}
% \RequirePackage{animate}

% tables
\usepackage{dcolumn}% Align table columns on decimal point
% \RequirePackage{array}
% \RequirePackage{longtable, lscape}
% \RequirePackage{multirow}
\RequirePackage{tabularx}
\RequirePackage{booktabs}


% source code
% \RequirePackage{listings}
% \lstset{language=bash,%
% basicstyle=\tiny\ttfamily\bfseries\color{Vermillion},%
% commentstyle=\color{Grey},
% showstringspaces=false,%
% breaklines=true,%
% frameround=tttt,%
% frame=single}

% make it gay
\RequirePackage{xcolor}
\definecolor{Orange}{cmyk}{0, 0.5, 1, 0} % appropriate set for colour-blind
\definecolor{SkyBlue}{cmyk}{0.8, 0, 0, 0}
\definecolor{BluishGreen}{cmyk}{0.97, 0, 0.75, 0}
\definecolor{Yellow}{cmyk}{0.1, 0.05, 0.9, 0}
\definecolor{Blue}{cmyk}{1, 0.5, 0, 0}
\definecolor{Vermillion}{cmyk}{0, 0.8, 1, 0}
\definecolor{ReddishPurple}{cmyk}{0.1, 0.7, 0, 0}
\definecolor{Grey}{cmyk}{0, 0, 0, 0.6}
\definecolor{Black}{cmyk}{0, 0, 0, 1}

% pdf hyperref functionality
\RequirePackage{hyperref}
\hypersetup{colorlinks=true}
\hypersetup{linkcolor=Blue, urlcolor=Blue, citecolor=Blue}

% draft stage only
\usepackage[export]{adjustbox}
\RequirePackage{printlen}
\RequirePackage{layouts}
\RequirePackage{blindtext}
%\usepackage[modulo, mathlines]{lineno}
%\linenumbers

% hack to fix correct line numbers with displaymath
% \RequirePackage{etoolbox}
% \makeatletter
% \newcommand*\linenomathpatch{\@ifstar{\linenomathpatch@AMS}{\linenomathpatch@}}
% \newcommand*\linenomathpatch@[1]{
%   \expandafter\pretocmd\csname #1\endcsname {\linenomathWithnumbers}{}{}
%   \expandafter\pretocmd\csname #1*\endcsname{\linenomathWithnumbers}{}{}
%   \expandafter\apptocmd\csname end#1\endcsname {\endlinenomath}{}{}
%   \expandafter\apptocmd\csname end#1*\endcsname{\endlinenomath}{}{}
% }
% \newcommand*\linenomathpatch@AMS[1]{
%   \expandafter\pretocmd\csname #1\endcsname {\linenomathWithnumbersAMS}{}{}
%   \expandafter\pretocmd\csname #1*\endcsname{\linenomathWithnumbersAMS}{}{}
%   \expandafter\apptocmd\csname end#1\endcsname {\endlinenomath}{}{}
%   \expandafter\apptocmd\csname end#1*\endcsname{\endlinenomath}{}{}
% }
% \let\linenomathWithnumbersAMS\linenomathWithnumbers
% \patchcmd\linenomathWithnumbersAMS{\advance\postdisplaypenalty\linenopenalty}{}{}{}
% \makeatother
% \linenomathpatch{equation}
% \linenomathpatch*{gather}
% \linenomathpatch*{multline}
% \linenomathpatch*{align}
% \linenomathpatch*{alignat}
% \linenomathpatch*{flalign}

